Safe Reinforcement Learning by Imagining the Near Future

Safe reinforcement learning is a promising path toward applying reinforcement learning algorithms to real-world problems, where suboptimal behaviors may lead to actual negative consequences. In this work, we focus on the setting where unsafe states can be avoided by planning ahead a short time into the future. In this setting, a model-based agent with a sufficiently accurate model can avoid unsafe states. We devise a model-based algorithm that heavily penalizes unsafe trajectories, and derive guarantees that our algorithm can avoid unsafe states under certain assumptions. Experiments demonstrate that our algorithm can achieve competitive rewards with fewer safety violations in several continuous control tasks.

==> 98-checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} In \Cref{sec:limitations}.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} In \Cref{sec:neg-social-impact}.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} \bibiL{Check}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{} \bibiL{check}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} In \Cref{sec:impl-details}.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} In \Cref{sec:impl-details}.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> 99-limitation.tex <==
\section{Limitations}
\label{sec:limitations}

\begin{itemize}
    \item The true $H^*$, if there even exists such an $H^*$ (it is hard to verify), is not known in general, forcing us to choose it as a hyperparameter.
    \item The model-based approach relies on the model making reasonably accurate predictions. We had trouble scaling our algorithm to tasks with higher-dimensional state spaces, where prediction is more challenging.
\end{itemize}

\section{Negative Social Impact}
\label{sec:neg-social-impact}
We believe that most of the impacts of this work are positive, but there are some risks:
\begin{itemize}
    \item Improved automation technology will likely lead to elimination of some kinds of jobs. (Although it may create others.)
    \item Labeling an algorithm as ``safe'' may lead people to trust it more than they otherwise would. It is important for practitioners of safe RL to understand the limitations of the algorithms they use.
\end{itemize}
